Data Acquisition for Improving Machine Learning Models

The vast advances in Machine Learning over the last ten years have been powered by the availability of suitably prepared data for training purposes. The future of ML-enabled enterprise hinges on data. As such, there is already a vibrant market offering data annotation services to tailor sophisticated ML models. In this paper, we present research on the practical problem of obtaining data in order to improve the accuracy of ML models. We consider an environment in which consumers query for data to enhance the accuracy of their models and data providers who possess data make them available for training purposes. We first formalize this interaction process laying out the suitable framework and associated parameters for data exchange. We then propose two data acquisition strategies that consider a trade-off between exploration during which we obtain data to learn about the distribution of a provider's data and exploitation during which we optimize our data inquiries utilizing the gained knowledge. In the first strategy, Estimation and Allocation, we utilize queries to estimate the utilities of various predicates while learning about the distribution of the provider's data; then we proceed to the allocation stage in which we utilize those learned utility estimates to inform our data acquisition decisions. The second algorithmic proposal, named Sequential Predicate Selection, utilizes a sampling strategy to explore the distribution of the provider's data, adaptively investing more resources to parts of the data space that are statistically more promising to improve overall model accuracy. We present a detailed experimental evaluation of our proposals utilizing a variety of ML models and associated real data sets exploring all applicable parameters of interest. We identify trade-offs and highlight the relative benefits of each algorithm to further optimize model accuracy.

==> reward.tex <==
\section{Utility Measurement}
\label{sec:utility_measurement}
Since re-training can only be conducted periodically during the transaction process, we need to estimate the potential performance gain a set of records $\mathcal{R}$ bring to $\mathcal{M}$ based on the state of $\mathcal{M}$ and characteristics of $\mathcal{R}$. Similar problems have been studied in the area of Active Learning (AL), where the two factors generally considered are uncertainty and diversity. However, there are two major aspects where AL differs from the problem studied in this paper, which prevents the applicability of the utility measurement proposed therein: (1) the features of all records are visible in AL tasks, and (2) the utility of a set of records is estimated without seeing their labels. In this section, we discuss how to quantify the utility for our problem considering the two factors.

Uncertainty mainly describes how much error $\mathcal{M}$ is likely to make when making predictions for $\mathcal{R}$. Since both the features and targets of records in $\mathcal{R}$ are available, quantifying the uncertainty is straightforward: we can directly utilize function $F$ to evaluate the performance of $\mathcal{M}$ and the value $F(\mathcal{M};\mathcal{R})$ can be used to indicate the uncertainty, denoted as $U(\mathcal{R})$.

Let $\mathcal{R}_{\mathcal{M}}$ be the records already seen by $\mathcal{M}$. Diversity describes the difference between the distribution of $\mathcal{R}_{\mathcal{M}}$ and the distribution of $\mathcal{R}$. We adopt a method widely used in areas including Information Theory \cite{DBLP:conf/iclr/Lopez-PazO17} and Transfer Learning \cite{DBLP:conf/cvpr/YanAF20} to quantify the diversity between $\mathcal{R}_{\mathcal{M}}$ and $\mathcal{R}$, with certain modifications to fit in our setting. The method consists of the following steps:
\begin{enumerate}
    \item View $\mathcal{R}_{\mathcal{M}}$ and $\mathcal{R}$ as two different classes;
    \item Train a classifier to discriminate records from both classes;
    \item Let $acc$ be the accuracy of the classifier on $\mathcal{R}$, then $acc$ is used as the indicator of the diversity, denoted as $D(\mathcal{R})$.
\end{enumerate}

The intuition behind the method is that, if $\mathcal{R}$ follows different distribution from $\mathcal{R}_{\mathcal{M}}$, then records belonging to $\mathcal{R}$ can be easily discriminated and $D(\mathcal{R})$ is high. On the other hand, if $\mathcal{R}$ and $\mathcal{R}_{\mathcal{M}}$ follow similar distribution, the two classes can hardly be discriminated and $D(\mathcal{R})$ is thus low. Note that we only consider the accuracy of the classifier on $\mathcal{R}$ because with diversity we measure how surprising $\mathcal{R}$ is given $\mathcal{R}_{\mathcal{M}}$ rather than the other way around. For example, assume that $\mathcal{R}\subset\mathcal{R}_{\mathcal{M}}$, then the diversity should be 0. However the accuracy on $\mathcal{R}_{\mathcal{M}}$ would be larger than 0 as $\mathcal{R}_{\mathcal{M}}\setminus\mathcal{R}$ can be discriminated from $\mathcal{R}$.

% We thus define the utility of $\mathcal{R}$, $utility(\mathcal{R})$, as the multiplication of $U(\mathcal{R})$ and $D(\mathcal{R})$:
% \begin{equation}
%     utility(\mathcal{R})=U(\mathcal{R})*D(\mathcal{R})
% \end{equation}

% Note that other forms of the utility function integrating factors besides uncertainty and diversity cooperate seamlessly with the methods proposed below.
We thus define the utility of $\mathcal{R}$, $utility(\mathcal{R})$, as a function of both $U(\mathcal{R})$ and $D(\mathcal{R})$:
\begin{equation}
    utility(\mathcal{R})=G(U(\mathcal{R}),D(\mathcal{R}))
\end{equation}

We experimentally study different forms of $G$ in Section x.
